The Clusters AgeS Experiment (CASE). III. Analysis of the Eccentric Eclipsing Binary V32 in the Globular Cluster NGC 6397

We present spectroscopic and photometric observations of the eclipsing binary V32 located in the central field of the globular cluster NGC 6397. The variable is a single-line spectroscopic binary with an orbital period of 9.8783d and a large eccentricity of e=0.32. Its systemic velocity (gamma=20.7 km/s) and metallicity ([Fe/H] -1.9) are both consistent with cluster membership. The primary component of the binary is located at the top of the main-sequence turn-off on the cluster color-magnitude diagram. Only a shallow primary eclipse is observed in the light curve. Based on stellar models for an age of 12Gyr and the mass-function derived from the radial velocity curve, we estimate the masses to be M_p=0.79 Msun and M_s=0.23 Msun. The light curve of V32 can be reproduced by adopting R_p=1.569 Rsun and R_s=0.236 Rsun for the radii and i=85.44 deg for the system inclination. The system geometry precludes observations of the secondary eclipse. The large eccentricity of the orbit is puzzling given that for metal poor, halo binaries the transition from circular to eccentric orbit occurs at an orbital period of about 20 days. We suppose that the orbit of V32 was modified relatively recently by dynamical interaction with other cluster star(s).An alternative explanation of the observed eccentricity calls for the presence of a third body in the system.

==> table_3_full.tex <==

\begin{deluxetable}{lcc}
\tablecolumns{3}
\tablewidth{0pt}
\tabletypesize{\small}
\tablecaption{$V$-band Photometric Observations of V32
\label{tab3}}
\tablehead{
\colhead{HJD}         &
\colhead{$V$}     &
\colhead{$\sigma_V$ }       \\
\colhead{(- 2450000)} &
\colhead{} &
\colhead{}      
}
\startdata  
2765.8121 16.128 0.008
2765.8209 16.134 0.008
2765.8277 16.128 0.008
2765.8371 16.126 0.008
2765.8677 16.125 0.008
2765.8894 16.129 0.008
2765.8966 16.122 0.008
2765.9061 16.129 0.008
2765.9128 16.127 0.008
2765.9294 16.131 0.008
2766.6934 16.130 0.006
2766.7008 16.129 0.006
2766.7215 16.130 0.007
2766.7288 16.124 0.006
2766.7353 16.124 0.006
2766.7455 16.128 0.006
2766.7497 16.127 0.006
2766.7537 16.126 0.006
2766.7603 16.119 0.006
2766.7638 16.130 0.006
2766.7675 16.126 0.006
2766.7725 16.129 0.006
2766.7766 16.128 0.007
2766.7805 16.131 0.006
2766.7845 16.130 0.006
2766.7884 16.126 0.006
2766.7919 16.128 0.006
2766.7963 16.130 0.006
2766.8031 16.124 0.007
2766.8067 16.126 0.007
2766.8102 16.126 0.007
2766.8142 16.129 0.006
2766.8181 16.128 0.006
2766.8219 16.129 0.006
2766.8256 16.126 0.006
2766.8291 16.131 0.006
2766.8326 16.129 0.006
2766.8361 16.128 0.006
2766.8397 16.126 0.006
2766.8433 16.123 0.006
2766.8470 16.131 0.006
2766.8509 16.127 0.006
2766.8545 16.124 0.006
2766.8588 16.132 0.006
2766.8624 16.129 0.006
2766.8666 16.124 0.006
2766.8707 16.129 0.006
2766.8748 16.128 0.006
2766.8786 16.123 0.006
2766.8867 16.124 0.006
2766.8907 16.126 0.006
2766.8946 16.128 0.006
2766.8986 16.130 0.007
2766.9028 16.121 0.007
2766.9075 16.123 0.006
2766.9124 16.123 0.007
2766.9168 16.126 0.006
2766.9218 16.127 0.007
2766.9282 16.126 0.006
2766.9301 16.125 0.007
2766.9355 16.127 0.007
2768.8077 16.130 0.007
2768.8132 16.127 0.009
2768.8182 16.125 0.008
2768.8235 16.132 0.009
2768.8291 16.130 0.009
2768.8346 16.126 0.008
2768.8396 16.125 0.006
2768.8479 16.124 0.008
2768.8560 16.127 0.008
2768.8903 16.125 0.008
2768.8974 16.126 0.008
3106.8613 16.126 0.006
3106.8659 16.130 0.006
3106.8702 16.134 0.006
3106.8744 16.126 0.006
3106.8782 16.129 0.007
3106.8823 16.128 0.007
3106.8869 16.129 0.008
3106.8912 16.131 0.008
3106.8957 16.128 0.008
3106.9004 16.126 0.008
3106.9048 16.129 0.008
3106.9097 16.125 0.008
3106.9142 16.129 0.008
3106.9186 16.129 0.008
3106.9228 16.131 0.008
3106.9270 16.127 0.009
3106.9307 16.128 0.010
3109.7934 16.154 0.006
3109.7970 16.154 0.006
3109.8009 16.156 0.006
3109.8044 16.156 0.006
3109.8084 16.154 0.006
3109.8120 16.155 0.006
3109.8179 16.152 0.006
3109.8230 16.153 0.006
3109.8269 16.159 0.006
3109.8308 16.154 0.006
3109.8346 16.156 0.006
3109.8396 16.155 0.006
3109.8451 16.155 0.006
3109.8495 16.152 0.006
3109.8556 16.152 0.006
3109.8610 16.154 0.006
3109.8653 16.154 0.006
3109.8701 16.150 0.006
3109.8746 16.145 0.006
3109.8785 16.144 0.006
3109.8835 16.140 0.006
3109.8883 16.137 0.006
3109.8943 16.136 0.006
3109.8991 16.131 0.006
3109.9039 16.130 0.006
3109.9080 16.128 0.006
3109.9120 16.127 0.006
3109.9161 16.124 0.006
3109.9208 16.130 0.006
3109.9249 16.129 0.006
3109.9285 16.124 0.007
3150.6334 16.128 0.009
3150.6483 16.126 0.009
3150.6532 16.128 0.008
3150.6582 16.126 0.008
3150.6622 16.131 0.008
3150.6720 16.128 0.008
3150.6758 16.126 0.008
3150.6854 16.125 0.008
3150.6898 16.125 0.008
3150.6938 16.129 0.009
3150.7052 16.125 0.009
3150.7292 16.123 0.009
3150.7344 16.129 0.009
3150.7382 16.117 0.008
3150.7478 16.128 0.009
3150.7531 16.123 0.008
3150.8320 16.132 0.009
3150.8455 16.131 0.009
3150.8502 16.126 0.008
3150.8606 16.126 0.009
3152.6580 16.128 0.007
3152.6633 16.128 0.007
3152.6678 16.127 0.007
3152.6721 16.128 0.007
3152.6818 16.129 0.007
3152.6860 16.129 0.007
3152.6904 16.125 0.007
3152.6944 16.127 0.007
3152.6984 16.132 0.007
3152.7014 16.130 0.007
3152.7095 16.127 0.007
3152.7136 16.129 0.007
3152.7175 16.129 0.007
3152.7212 16.130 0.007
3152.7302 16.129 0.007
3152.7343 16.130 0.007
3152.7381 16.131 0.007
3152.7419 16.128 0.008
3152.7511 16.130 0.007
3152.7551 16.121 0.008
3152.7592 16.128 0.008
3152.7634 16.130 0.008
3152.7723 16.129 0.008
3152.7764 16.130 0.007
3152.7806 16.127 0.007
3152.7836 16.127 0.007
3152.7911 16.132 0.007
3152.7950 16.136 0.007
3152.7990 16.131 0.007
3152.8026 16.122 0.007
3152.8127 16.129 0.007
3152.8167 16.129 0.007
3152.8204 16.129 0.007
3152.8315 16.131 0.007
3152.8354 16.131 0.007
3152.8397 16.133 0.007
3152.8442 16.131 0.008
3152.8527 16.130 0.008
3152.8573 16.131 0.007
3152.8629 16.128 0.008
3152.8729 16.126 0.008
3152.8773 16.130 0.009
3153.8102 16.135 0.008
3153.8264 16.132 0.008
3153.8300 16.126 0.008
3154.9210 16.128 0.008
3154.9250 16.128 0.008
3202.6396 16.126 0.009
3202.6483 16.128 0.009
3202.6568 16.126 0.009
3202.6735 16.135 0.012
3202.6916 16.129 0.009
3202.7237 16.132 0.009
3202.7582 16.130 0.009
3203.4768 16.132 0.009
3203.4834 16.126 0.006
3203.4882 16.132 0.006
3203.4958 16.123 0.006
3203.4989 16.133 0.006
3203.5053 16.130 0.006
3203.5084 16.132 0.006
3203.5204 16.131 0.006
3203.5237 16.129 0.006
3203.5324 16.131 0.006
3203.5355 16.133 0.006
3203.5424 16.125 0.006
3203.5455 16.131 0.006
3203.5538 16.128 0.006
3203.5569 16.129 0.006
3203.5635 16.128 0.006
3203.5666 16.134 0.006
3203.5731 16.128 0.006
3203.5763 16.130 0.006
3203.5824 16.126 0.006
3203.5855 16.129 0.006
3203.5922 16.132 0.006
3203.5953 16.127 0.006
3203.6036 16.130 0.006
3203.6071 16.126 0.006
3203.6156 16.129 0.006
3203.6187 16.130 0.006
3203.6251 16.126 0.006
3203.6282 16.129 0.006
3203.6349 16.126 0.006
3203.6380 16.127 0.006
3203.6446 16.130 0.006
3203.6478 16.132 0.006
3203.6555 16.127 0.006
3203.6589 16.126 0.006
3203.6651 16.128 0.006
3203.6779 16.129 0.006
3203.6810 16.130 0.006
3203.6880 16.129 0.006
3203.6911 16.134 0.006
3203.6975 16.133 0.006
3203.7006 16.131 0.006
3203.7070 16.129 0.006
3203.7101 16.130 0.006
3203.7168 16.131 0.006
3203.7199 16.130 0.006
3203.7273 16.126 0.006
3203.7304 16.133 0.006
3203.7374 16.129 0.006
3203.7406 16.124 0.006
3203.7478 16.125 0.006
3203.7509 16.130 0.006
3203.7576 16.126 0.006
3203.7607 16.132 0.006
3203.7672 16.122 0.006
3203.7703 16.132 0.006
3204.5906 16.127 0.006
3204.5938 16.129 0.006
3204.6014 16.129 0.006
3204.6045 16.128 0.006
3204.6114 16.132 0.006
3204.6145 16.127 0.006
3204.6225 16.129 0.006
3204.6256 16.127 0.006
3204.6329 16.124 0.006
3204.6361 16.128 0.006
3204.6431 16.130 0.006
3204.6464 16.126 0.006
3204.6529 16.125 0.006
3204.6560 16.131 0.006
3204.6637 16.134 0.006
3204.6668 16.130 0.006
3204.6758 16.129 0.006
3204.6789 16.130 0.006
3204.6854 16.131 0.006
3204.6886 16.133 0.006
3204.6953 16.132 0.006
3204.6984 16.129 0.006
3204.7055 16.131 0.006
3204.7087 16.133 0.006
3204.7160 16.126 0.006
3204.7191 16.130 0.006
3204.7257 16.131 0.006
3204.7288 16.130 0.006
3204.7352 16.129 0.006
3204.7383 16.127 0.006
3204.7453 16.129 0.006
3204.7487 16.129 0.006
3204.7570 16.131 0.007
3204.7604 16.127 0.007
3204.7678 16.132 0.006
3204.7710 16.129 0.007
3206.4773 16.135 0.008
3206.6976 16.132 0.007
3206.7025 16.125 0.008
3206.7139 16.131 0.008
3206.7174 16.132 0.008
3206.7284 16.131 0.009
3206.7339 16.130 0.009
3206.7424 16.129 0.009
4295.4611 16.132 0.011
4295.4654 16.131 0.010
4295.4706 16.129 0.010
4295.4754 16.131 0.010
4295.4801 16.130 0.010
4295.4850 16.128 0.009
4295.4893 16.133 0.010
4295.4929 16.132 0.009
4295.4966 16.131 0.009
4295.5010 16.133 0.009
4295.5056 16.126 0.009
4295.5100 16.128 0.009
4295.5139 16.126 0.009
4295.5181 16.133 0.009
4295.5220 16.129 0.009
4295.5264 16.128 0.009
4295.5310 16.125 0.009
4295.5349 16.129 0.009
4295.5382 16.126 0.009
4295.5417 16.128 0.009
4295.5482 16.133 0.010
4295.5543 16.137 0.010
4295.5597 16.131 0.010
4295.5643 16.129 0.009
4302.6105 16.133 0.008
4334.6339 16.126 0.100
4334.6403 16.132 0.100
4334.6484 16.129 0.100
4334.6551 16.130 0.100
4335.5204 16.129 0.100
4335.5245 16.126 0.100
4335.5286 16.132 0.100
4335.5361 16.128 0.100
4335.5405 16.130 0.100
4339.6448 16.130 0.100
4340.5589 16.125 0.100
4340.5732 16.133 0.100
4340.5812 16.129 0.100
4340.5831 16.127 0.100
4340.5893 16.131 0.100
4340.5912 16.130 0.100
\enddata
\end{deluxetable}

